Simulating Chemical Abundances in the Circumstellar Nebula of the Late Stage Binary RY Scuti

RY Scuti, thought to be a Wolf-Rayet (WR) progenitor, is a massive, post-main-sequence, binary star system undergoing Roche lobe overflow (RLOF). SOFIA (+FORCAST) spectroscopy of the inner, ionized region of RY Scuti's double ringed toroidal nebula affirms the previous detection of the well-studied 12.81 $\mu$m Ne II forbidden transition and reveals four distinct emission lines, including three previously undetected transitions, S III, Fe III, and S III. Cloudy photoionization modeling of the four neon, sulfur, and iron lines was performed to derive fractional abundances (log($\frac{X}{H}$)) of neon at -3.19 $\pm$ 0.0251, sulfur at -3.76 $\pm$ 0.0487, and iron at -2.23 $\pm$ 0.0286. All three species are overabundant with respect to fiducial solar chemical abundances, especially iron. Our analysis suggests that the outer envelope of the primary star in the RY Scuti system is being stripped away via RLOF, leaving helium-rich and hydrogen-poor material visible to observation. This material also exhibits elevated neon, sulfur, and iron fractional abundances, consistent with RY Scuti evolving toward a WR object.

==> Notes/aasGuide.tex <==
% STYLE GUIDE   
% https://journals.aas.org/aas-style-guide/#1590154699721-1360f383-a572

% GRAPHICS GUIDE
% https://journals.aas.org/graphics-guide/

% DATA GUIDE
% https://journals.aas.org/data-guide/

% FULL AUTHOR GUIDE
% https://journals.aas.org/aastexguide/

==> Notes/aastexNotes.tex <==
%% AASTeX requires revtex4-1.cls and other external packages such as
%% latexsym, graphicx, amssymb, longtable, and epsf.  Note that as of 
%% Oct 2020, APS now uses revtex4.2e for its journals but remember that 
%% AASTeX v6+ still uses v4.1. All of these external packages should 
%% already be present in the modern TeX distributions but not always.
%% For example, revtex4.1 seems to be missing in the linux version of
%% TexLive 2020. One should be able to get all packages from www.ctan.org.
%% In particular, revtex v4.1 can be found at 
%% https://www.ctan.org/pkg/revtex4-1.

%% The first piece of markup in an AASTeX v6.x document is the \documentclass
%% command. LaTeX will ignore any data that comes before this command. The 
%% documentclass can take an optional argument to modify the output style.
%% The command below calls the preprint style which will produce a tightly 
%% typeset, one-column, single-spaced document.  It is the default and thus
%% does not need to be explicitly stated.

%% ------------------------------------------------------------------------------

%% The default is a single spaced, 10 point font, single spaced article.
%% There are 5 other style options available via an optional argument. They
%% can be invoked like this:
%%
%% \documentclass[arguments]{aastex631}
%% 
%% where the layout options are:
%%
%%  twocolumn   : two text columns, 10 point font, single spaced article.
%%                This is the most compact and represent the final published
%%                derived PDF copy of the accepted manuscript from the publisher
%%  manuscript  : one text column, 12 point font, double spaced article.
%%  preprint    : one text column, 12 point font, single spaced article.  
%%  preprint2   : two text columns, 12 point font, single spaced article.
%%  modern      : a stylish, single text column, 12 point font, article with
%% 		  wider left and right margins. This uses the Daniel
%% 		  Foreman-Mackey and David Hogg design.
%%  RNAAS       : Supresses an abstract. Originally for RNAAS manuscripts 
%%                but now that abstracts are required this is obsolete for
%%                AAS Journals. Authors might need it for other reasons. DO NOT
%%                use \begin{abstract} and \end{abstract} with this style.
%%
%% Note that you can submit to the AAS Journals in any of these 6 styles.
%%
%% There are other optional arguments one can invoke to allow other stylistic
%% actions. The available options are:
%%
%%   astrosymb    : Loads Astrosymb font and define \astrocommands. 
%%   tighten      : Makes baselineskip slightly smaller, only works with 
%%                  the twocolumn substyle.
%%   times        : uses times font instead of the default
%%   linenumbers  : turn on lineno package.
%%   trackchanges : required to see the revision mark up and print its output
%%   longauthor   : Do not use the more compressed footnote style (default) for 
%%                  the author/collaboration/affiliations. Instead print all
%%                  affiliation information after each name. Creates a much 
%%                  longer author list but may be desirable for short 
%%                  author papers.
%% twocolappendix : make 2 column appendix.
%%   anonymous    : Do not show the authors, affiliations and acknowledgments 
%%                  for dual anonymous review.
%%
%% these can be used in any combination, e.g.
%%
%% \documentclass[twocolumn,linenumbers,trackchanges]{aastex631}
%%
%% AASTeX v6.* now includes \hyperref support. While we have built in specific
%% defaults into the classfile you can manually override them with the
%% \hypersetup command. For example,
%%
%% \hypersetup{linkcolor=red,citecolor=green,filecolor=cyan,urlcolor=magenta}
%%
%% will change the color of the internal links to red, the links to the
%% bibliography to green, the file links to cyan, and the external links to
%% magenta. Additional information on \hyperref options can be found here:
%% https://www.tug.org/applications/hyperref/manual.html#x1-40003
%%
%% Note that in v6.3 "bookmarks" has been changed to "true" in hyperref
%% to improve the accessibility of the compiled pdf file.
%%
%% If you want to create your own macros, you can do so
%% using \newcommand. Your macros should appear before
%% the \begin{document} command.
%%

%% ------------------------------------------------------------------------------

%% Reintroduced the \received and \accepted commands from AASTeX v5.2
%\received{March 1, 2021}
%\revised{April 1, 2021}
%\accepted{\today}

%% Command to document which AAS Journal the manuscript was submitted to.
%% Adds "Submitted to " the argument.
%\submitjournal{PSJ}

%% For manuscript that include authors in collaborations, AASTeX v6.31
%% builds on the \collaboration command to allow greater freedom to 
%% keep the traditional author+affiliation information but only show
%% subsets. The \collaboration command now must appear AFTER the group
%% of authors in the collaboration and it takes TWO arguments. The last
%% is still the collaboration identifier. The text given in this
%% argument is what will be shown in the manuscript. The first argument
%% is the number of author above the \collaboration command to show with
%% the collaboration text. If there are authors that are not part of any
%% collaboration the \nocollaboration command is used. This command takes
%% one argument which is also the number of authors above to show. A
%% dashed line is shown to indicate no collaboration. This example manuscript
%% shows how these commands work to display specific set of authors 
%% on the front page.
%%
%% For manuscript without any need to use \collaboration the 
%% \AuthorCollaborationLimit command from v6.2 can still be used to 
%% show a subset of authors.
%
%\AuthorCollaborationLimit=2
%
%% will only show Schwarz & Muench on the front page of the manuscript
%% (assuming the \collaboration and \nocollaboration commands are
%% commented out).
%%
%% Note that all of the author will be shown in the published article.
%% This feature is meant to be used prior to acceptance to make the
%% front end of a long author article more manageable. Please do not use
%% this functionality for manuscripts with less than 20 authors. Conversely,
%% please do use this when the number of authors exceeds 40.
%%
%% Use \allauthors at the manuscript end to show the full author list.
%% This command should only be used with \AuthorCollaborationLimit is used.

%% The following command can be used to set the latex table counters.  It
%% is needed in this document because it uses a mix of latex tabular and
%% AASTeX deluxetables.  In general it should not be needed.
%\setcounter{table}{1}

%% ------------------------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% The following section outlines numerous optional output that
%% can be displayed in the front matter or as running meta-data.
%%
%% If you wish, you may supply running head information, although
%% this information may be modified by the editorial offices.
%% \shorttitle{AASTeX v6.31 Sample article}
%% \shortauthors{Schwarz et al.}
%%
%% You can add a light gray and diagonal water-mark to the first page 
%% with this command:
%% \watermark{text}
%% where "text", e.g. DRAFT, is the text to appear.  If the text is 
%% long you can control the water-mark size with:
%% \setwatermarkfontsize{dimension}
%% where dimension is any recognized LaTeX dimension, e.g. pt, in, etc.
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ------------------------------------------------------------------------------

%% A significant change from earlier AASTEX versions is in the structure for 
%% calling author and affiliations. The change was necessary to implement 
%% auto-indexing of affiliations which prior was a manual process that could 
%% easily be tedious in large author manuscripts.
%%
%% The \author command is the same as before except it now takes an optional
%% argument which is the 16 digit ORCID. The syntax is:
%% \author[xxxx-xxxx-xxxx-xxxx]{Author Name}
%%
%% This will hyperlink the author name to the author's ORCID page. Note that
%% during compilation, LaTeX will do some limited checking of the format of
%% the ID to make sure it is valid. If the "orcid-ID.png" image file is 
%% present or in the LaTeX pathway, the OrcID icon will appear next to
%% the authors name.
%%
%% Use \affiliation for affiliation information. The old \affil is now aliased
%% to \affiliation. AASTeX v6.31 will automatically index these in the header.
%% When a duplicate is found its index will be the same as its previous entry.
%%
%% Note that \altaffilmark and \altaffiltext have been removed and thus 
%% can not be used to document secondary affiliations. If they are used latex
%% will issue a specific error message and quit. Please use multiple 
%% \affiliation calls for to document more than one affiliation.
%%
%% The new \altaffiliation can be used to indicate some secondary information
%% such as fellowships. This command produces a non-numeric footnote that is
%% set away from the numeric \affiliation footnotes.  NOTE that if an
%% \altaffiliation command is used it must come BEFORE the \affiliation call,
%% right after the \author command, in order to place the footnotes in
%% the proper location.
%%
%% Use \email to set provide email addresses. Each \email will appear on its
%% own line so you can put multiple email address in one \email call. A new
%% \correspondingauthor command is available in V6.31 to identify the
%% corresponding author of the manuscript. It is the author's responsibility
%% to make sure this name is also in the author list.
%%
%% While authors can be grouped inside the same \author and \affiliation
%% commands it is better to have a single author for each. This allows for
%% one to exploit all the new benefits and should make book-keeping easier.
%%
%% If done correctly the peer review system will be able to
%% automatically put the author and affiliation information from the manuscript
%% and save the corresponding author the trouble of entering it by hand.

%\correspondingauthor{August Muench}
%\email{greg.schwarz@aas.org, gus.muench@aas.org}

%% Note that the \and command from previous versions of AASTeX is now
%% depreciated in this version as it is no longer necessary. AASTeX 
%% automatically takes care of all commas and "and"s between authors names.

%% ------------------------------------------------------------------------------

%% AASTeX 6.31 has the new \collaboration and \nocollaboration commands to
%% provide the collaboration status of a group of authors. These commands 
%% can be used either before or after the list of corresponding authors. The
%% argument for \collaboration is the collaboration identifier. Authors are
%% encouraged to surround collaboration identifiers with ()s. The 
%% \nocollaboration command takes no argument and exists to indicate that
%% the nearby authors are not part of surrounding collaborations.

%% ------------------------------------------------------------------------------

%% Keywords should appear after the \end{abstract} command. 
%% The AAS Journals now uses Unified Astronomy Thesaurus concepts:
%% https://astrothesaurus.org
%% You will be asked to selected these concepts during the submission process
%% but this old "keyword" functionality is maintained in case authors want
%% to include these concepts in their preprints.
%% \keywords{Classical Novae (251) --- Ultraviolet astronomy(1736) --- History of astronomy(1868) --- Interdisciplinary astronomy(804)}

%% From the front matter, we move on to the body of the paper.
%% Sections are demarcated by \section and \subsection, respectively.
%% Observe the use of the LaTeX \label
%% command after the \subsection to give a symbolic KEY to the
%% subsection for cross-referencing in a \ref command.
%% You can use LaTeX's \ref and \label commands to keep track of
%% cross-references to sections, equations, tables, and figures.
%% That way, if you change the order of any elements, LaTeX will
%% automatically renumber them.
%%
%% We recommend that authors also use the natbib \citep
%% and \citet commands to identify citations.  The citations are
%% tied to the reference list via symbolic KEYs. The KEY corresponds
%% to the KEY in the \bibitem in the reference list below. 

==> notes.tex <==
Major concerns:
1.) - line 6: "post-main-sequence, overcontact binary star system undergoing Roche lobe overflow (RLOF)" - This seems a bit confusing to me. If its an overcontact binary then both components should be overfilling their roche lobes. Roche lobe overflow to me usually refers to systems where only one component is filling its roche lobe and transferring mass to its component, unless you are implying that it is overflowing through L2. In the case of overcontact systems, even if there is net mass transfer through the bridge, the two components should share a common potential unless the system is in a transitionary stage which should be evolving on the thermal timescale at most. Could you please clarify which of these scenarios is relevant to this system in the text?
-Indeed, RY Scuti’s RLOF is occurring when only one star (the mass donor) of the binary is expanding to fill its Roche lobe, not double component mass transfer. We agree with the referee that the phrase “overcontact” is not an accurate representation of what is occurring in the system and have therefore removed all mentions of the phrase from the manuscript.

2.) - line 112: "including five new lines (S III, Fe III, Fe III, S III, and Ne III) not identified in previous RY Scuti spectra" - The wavelengths of these lines should be given here. That said, given that some of these are eliminated in the telluric correction, I don't understand why they are cited here. If the data is deemed of insufficient quality in these regions, then how reliable are these line identifications? Are these real or are they contaminated by telluric lines? Also what is the S/N of these detections? Are they significant?
-All references to the lines contaminated by telluric noise are removed from the paper, both in the text and in Figure 1, as the referee correctly points out, these lines are contaminated and deemed unworthy of analysis. 
-Wavelengths for the three new lines are now included in lines 120-121 and are marked in red. We used Specutils to calculate the S/N of each detection, and these are now reported in Table 1 in a new column to the right of the line flux, marked in red.


3.) - line 271: "during the χ2 minimization process" - How was the chi square minimization conducted? Was this a grid based approach, or MCMC, or was a minimization routine used? I see that a MC simulation was used to get the errors, but how was the best fit solution actually determined? Were the abundances derived for each line individually or was a fit obtained for the all abundances simultaneously? If so, were the lines weighted differently or were all weighted the same? Were the abundances the only free parameter allowed in the MC simulation or were parameters allowed to vary as well? Also how does the up to 1 magnitude of error on the continuum affect the abundances that are derived? From the analysis methods described, it doesn't seem that this error in the continuum is propagated to the abundance errors.
-A minimization routine was used to determine the best fit solution, specifically the Powell method using “scipy.optimize.minimize”. The abundances for each line change with each minimization iteration, but the actual chi square is the summation of the offsets in the lines, so the fit is obtained for all lines and abundances simultaneously. The lines were all weighted the same. The abundances were the only free parameter allowed in the MC simulation. Lines 264-267 and 287-289 were added to the paper to clarify these points, and are set in red.
-Since the free-free continuum was resistant to changes in Ne, S, and Fe, the difference between the modeled and radio extrapolated free-free continuum is not extrapolated in the errors for each of those three abundances. Discussion of the limitations in the free-free fitting method is included in lines 515-522.

4.) - Figure 3: you use the radio extrapolated free-free continuum to constrain the cloudy models, but given the large difference in the slope between the extrapolated radio continuum and the cloudy one, how strong is the disagreement in the opposite direction? As in, if you extrapolate the cloudy continuum back to the radio, how many orders of magnitude are you off? Also, the difference in the slopes should be discussed in the text. Was there no way to match both the slope and the extrapolated continuum from the radio?
-We fixed the slope issue, the two slopes are now identical so there is no major offset between the difference in the IR versus the difference in the radio. Since the slopes now match, we will not include a discussion about how the two were different.

5.) - Figure 4: you plot the integrated line intensities and the line ratios as a function of wavelength which doesn't have any meaning in this context. This is especially egregious in the right figure where a line is plotted, which implies that this ratios will hold for the wavelength regions covered by the line. Given that these are individual line ratios, the wavelength dependence is meaningless and misleading. From your plot as it is now, it implies that at 21 um for example, a line ratio of ~0.3 is expected, but given that there is no line observed at 21um this does not make any sense. For both of these, please remove wavelength from the x-axis and instead display these with an arbitrary x-axis. Also, please label the lines with their ionization state and wavelength so they can be more easily identified and discussed (e.g., Ne II λ12.83 or something similar). Furthermore, in the right panel, you can calculate the observed line ratio error bars through error propagation. That said, the plot would be much more informative if the observed line ratios were plotted as points with error bars and the best fit model was also plotted as a point with an error bar. If you still wish to display the MC results, these can still be plotted with lines in addition to the best fit point and errorbar, but again, the x-axis should be arbitrary units and not wavelength in this case.
-Indeed, the right panel of FIgure 4 is misleading as it indicates a wavelength dependence in the line ratios that does not exist. Since 1) the line ratios in the right panel are simply a different way to visualize the agreement between the lines which has already been illustrated in the left panel and 2) all of the MC results are encoded into and shown in the error bars of the simulated line intensities, the right panel of Figure 4 is unnecessary and has therefore been removed. The Figure 4 caption has been updated accordingly.

6.) - line 427: "While these simulations provided the desired result, the accompanying χ 2 value was larger than the χ 2 value for the best fit chemical abundances. Those models were therefore rejected." - You can adjust the weighting so that at least the breadth of each line is accounted for and this should allow for better agreement with the error bars. Usually when fitting spectra, reduced chi square is used, which would account for this as each wavelength point would contribute to the number of degrees of freedom and therefore weighs the lines accordingly. In this case, since you aren't fitting the lines directly but only the line strengths, this information appears to be lost.
-For a static resolution in Cloudy, the wavelengths of the output spectrum do not change from iteration to iteration, even if the chemical abundances do, meaning the thicknesses/line breadths and therefore the FWHM of each line are static. Thus, the FWHM is, at least for our simulation, not a useful parameter to include in the minimization routine since it does not change from simulation to simulation. This determination is discussed in lines 270-276. However, as the referee points out, FWHM is often a useful spectroscopic quantity, so we have therefore computed it for both the SOFIA observed lines and the simulated best fit Cloudy lines. The values are reported in Tables 1 and 4 respectively.

7.) -line 497: you mention that the abundances can't be compared directly because the star is partially stripped, but what about the line ratios? How do these compare with the solar ratios? Are these consistent? Given the levels of enhancement for iron (112x solar) and neon (2.5x solar) it seems that you would need vastly different levels of hydrogen depletion to explain each of these abundances, so I suspect that more is going on here than just simply hydrogen depletion.
-Indeed, the chemical abundances are not uniformly enriched and so their elevation cannot solely be attributed to hydrogen depletion alone. Some other enrichment factor must be at play. The discussion section, specifically lines 499-505, was edited to include this statement.

Minor concerns:
1.) -line 12: "of neon at at" - remove second "at"
-Removed, phrase set in red
2.) -line 114: "using the 4".7 slit" - is this written correctly? Should it be 4.7"?
-4”.7 is standard for AJ publications, not 4.7”. For example:          https://ui.adsabs.harvard.edu/abs/2024AJ....168...69Z/abstract, page 7, bottom left paragraph
3.) - line 233: "purple line in right panel of Figure 3" - The line is green not purple.
-Changed “purple” to “green”, word “green” set in red
4.) - line 282: Table 4 is referred to before Table 3 in the text.
-Table order switched so first reference to each table occurs in ascending numeric order
5.) - line 289: "to to determine" - remove second "to"
-Removed, phrase set in red
6.) - line 414 and throughout the text in other places: "ionic species" - change to "ionization state"
-Changes made to all instances of this phrase, all phrases set in red
7.) - line 536: "using a more robust fitting technique other than χ 2 minimization, such as least squares fitting." - the fitting technique would be whatever method you use to minimize chi square (I don't believe this was specified in the text as I pointed out above). I think you mean a more robust goodness of fit metric (chi square, least squares, log likelihood, etc.) In this case, least squares is not necessarily more robust than chi square but log likelihood is statistically more general and a better option however.
-Changed “lease squares fitting” to “log likelihood”, set in red

